Character-Centric Understanding of Animated Movies

Animated movies are captivating for their unique character designs and imaginative storytelling, yet they pose significant challenges for existing recognition systems. Unlike the consistent visual patterns detected by conventional face recognition methods, animated characters exhibit extreme diversity in their appearance, motion, and deformation. In this work, we propose an audio-visual pipeline to enable automatic and robust animated character recognition, and thereby enhance character-centric understanding of animated movies. Central to our approach is the automatic construction of an audio-visual character bank from online sources. This bank contains both visual exemplars and voice (audio) samples for each character, enabling subsequent multi-modal character recognition despite long-tailed appearance distributions. Building on accurate character recognition, we explore two downstream applications: Audio Description (AD) generation for visually impaired audiences, and character-aware subtitling for the hearing impaired. To support research in this domain, we introduce CMD-AM, a new dataset of 75 animated movies with comprehensive annotations. Our character-centric pipeline demonstrates significant improvements in both accessibility and narrative comprehension for animated content over prior face-detection-based approaches. For the code and dataset, visit https://www.robots.ox.ac.uk/~vgg/research/animated_ad/.

==> sections/X_not_used.tex <==
% the introduction. 


% A key enabler of such understanding is accurate character recognition. However, characters in animated movies appear in diverse forms: some resemble humans, while others exhibit abstract or imaginative designs. This long-tailed distribution of appearances poses a significant challenge for recognition methods.



% az comment:
% somewhere we should describe the 2-stage AD pipeline, to make it self-contained.
% "these two methods require characters" -- that's how this paper is about. 

% Teaser:
% pipeline inspired from "Emotion Recognition in Speech using
% Cross-Modal Transfer in the Wild".
% video coming in, show the key components, can have interaction between blocks.

% To some extend this maps to the sections -- can guide reader to read the papers.

% In figures, show one level up. Leave the method name in the implementation details.

% Frame visualization, also make clearer. 

% Dataset visualization as well, it is a good contribution. 

% Table 1, give a name of the dataset: Anima-xx. 

% Previous methods don't work -- show a table on this. 
% e.g. Face regocnition performance, 
% AD performance, 
% diarization performance, 
% audio-visual character recognition performance?

% update: visual char recog of characters, audio char recog of characters, diarization. 

% Feels like visual prompting detail is an important detail should be in the method, maybe sec 5.x. 
